Context-aware learning for generative models

This work studies the class of algorithms for learning with side-information that emerge by extending generative models with embedded context-related variables. Using finite mixture models (FMM) as the prototypical Bayesian network, we show that maximum-likelihood estimation (MLE) of parameters through expectation-maximization (EM) improves over the regular unsupervised case and can approach the performances of supervised learning, despite the absence of any explicit ground truth data labeling. By direct application of the missing information principle (MIP), the algorithms' performances are proven to range between the conventional supervised and unsupervised MLE extremities proportionally to the information content of the contextual assistance provided. The acquired benefits regard higher estimation precision, smaller standard errors, faster convergence rates and improved classification accuracy or regression fitness shown in various scenarios, while also highlighting important properties and differences among the outlined situations. Applicability is showcased with three real-world unsupervised classification scenarios employing Gaussian Mixture Models. Importantly, we exemplify the natural extension of this methodology to any type of generative model by deriving an equivalent context-aware algorithm for variational autoencoders (VAs), thus broadening the spectrum of applicability to unsupervised deep learning with artificial neural networks. The latter is contrasted with a neural-symbolic algorithm exploiting side-information.

==> sections/discriminative_discussion.tex <==
Another issue can be raised regarding the possibility to apply the proposed
framework on discriminative models. Although such evaluation is out of the scope
of this work, it is worth to discuss the different possibilities. Discriminative
modeling would imply reversing the dependence relation between the latent class
variables $z$ and the observed samples $\bs{x}$ in Figure~\ref{fig:model} to
directly model the conditional distribution $p(z|x)$. Algorithm \emph{DCA} can
be applied in the exact same fashion for discriminative models replacing the
marginal likelihood objective with the conditional one, although it will most
likely suffer the same shortcomings determined here. The exact formulation of
algorithms \emph{CA} and \emph{WCA}, being instances of EM--MLE, are bound to
optimization of the marginal likelihood and generative modeling and cannot be
extended in a straightforward manner to discriminative modeling. One possibility
is to exploit the analogy of our framework to the Posterior Regularization
scheme explained in Appendix~\ref{app:pr}, deriving an algorithm similar to
\emph{CA} and \emph{WCA} for discriminative models, as presented in
\citep[Section~2.8]{Ganchev10}. Albeit this will lead to an iterative algorithm
akin to EM for discriminative models exploiting context, it cannot be
equivalently derived through direct probabilistic modeling and exploitation of
internal model features, as in the generative case presented here. Another
possibility is to provide the versions of the algorithms \emph{CA} and
\emph{WCA} for the case of Maximum Conditional Likelihood (MCL) estimation, as
described in the seminal thesis of \citet{Jebara02}. By means of the same
principles applied here, this alternative objective should yield similar
benefits as those shown here for standard ML estimation, what remains of course
to be shown in practice. Even so, context--aware MCL would lose much of the
simplicity and intuitiveness that makes the algorithms presented here
particularly attractive. Last but not least, one can also envision the
straightforward implementation of a combination of generative and discriminative
modeling through mixtures of discriminative models (mixtures of experts),
preserving all the favorable properties of the proposed algorithms; it is easy
to show that our algorithms will behave similarly in a mixture of logistic
regressions scenario, in the same fashion that the demonstrated mixture of
linear regressions scenario does not loose the favorable properties compared to
mixtures of normal or Maxwell--Boltzmann distributions.


==> sections/results_longBCI.tex <==
In this section, we provide theoretical insights on how the proposed
context--aware methods improve FMM parameter estimation and establish their
connection to the missing information principle. We then present estimation
fitness, standard error and convergence rate results in various FMM parameter
estimation scenarios. Finally, classification results with the \emph{CA} method
are presented in an online--learning problem in brain--computer interaction.

\subsection{Likelihood landscapes}
\label{subsec:lik}

\begin{figure}[h!]
  \centering
  \includegraphics[width=\textwidth]{img/Figure1.pdf}
  \caption{(a) $logL(\mu_1)$ (solid lines) and
    $Q(\mu_1,\hat{\mu_1}^0)+H(\hat{\mu_1}^0,\hat{\mu_1}^0)$ (at first EM
    iteration, dashed lines) for various estimation methods as color--coded in
    the legend in a two--mixture, univariate Gaussian mixture model (see text).
    \emph{CAE} refers to method \emph{CA} with ignorant context (0 negentropy)
    and \emph{CA}, \emph{WCA} and \emph{DCA} are shown for contextual negentropy
    of 0.7. ML estimates after convergence shown with `x' and estimates after
    the first iteration in `o'.  (b) Incomplete--data log--likelihoods
    $logL(\mu_1)$ in the same problem as in (a) for \emph{US} (red solid) and
    various contextual negentropy levels as shown in the legend for \emph{CA}
    (blue) and \emph{WCA} (green). See section \ref{subsec:lik}.}
  \label{fig:liks}
\end{figure}

In order to intuitively demonstrate the effects of the proposed methods, we show
in Figure~\ref{fig:liks}a the incomplete--data log--likelihoods $logL(\mu_1)$
and the intermediate objectives maximized at the first M--step (complete--data
log--likelihood expectations plus the latent data entropy)
$Q(\mu_1,\hat{\mu_1}^0)+H(\hat{\mu_1}^0,\hat{\mu_1}^0)$ (see Appendix
\ref{app:proofs}) for a two--mixture of univariate Gaussians problem where only
$\mu_1$ is estimated starting from $\hat{\mu_1}^0=2$ and the rest of the
parameters are fixed to $\pi_1=0.1,\mu_2=1,s_1=0.5,s_2=3$. Estimation is based
on $N=100$ samples randomly generated from the above distribution using
$\mu_1=0$ (true parameter value). The above artificial setting is selected
because it generally leads to multiple local maxima (when $N$ is small) with a
maximum close to the true parameter value, which is not necessarily the global
maximum.

The first thing to note is that the intermediate objectives
$Q(\mu_1,\hat{\mu_1}^0)+H(\hat{\mu_1}^0,\hat{\mu_1}^0)$ (the results of the
first E--step of each method), like EM theory dictates, are tangent to the
respective complete--data log--likelihoods $logL(\mu_1)$ at the initial estimate
$\hat{\mu_i}^0=2$ having the same gradient as the corresponding $logL(\mu_1)$,
and thus they form a lower bound of $logL(\mu_1)$ which is maximized at the
first M--step to yield new estimates $\hat{\mu_1}^1$ (circles `o' in Figure
\ref{fig:liks}a). Besides illustrating the sanity of the methods, it is shown
that against initial intuition, context--aware methods do not simply alter the
E--step formulation; the latter is actually the result of forming a new
incomplete--data log--likelihood $L(\theta)$, different from that of the
``regular" \emph{US} method, as shown in Table \ref{tab:methods}. In fact, in
the illustrated example, the new estimates $\hat{\mu_1}^1$ for \emph{CA, WCA,
CAE} lead (naturally) to a higher point in their own respective $logL(\mu_1)$
curve than $\hat{\mu_1}^0$, but to a slightly lower point of $logL(\mu_1)$
corresponding to \emph{US} (solid red line).

The benefits of these methods (in case of ``correct" context as in the example)
come as a result of the features of the contextually modified $logL(\theta)$.
One can see that besides a vertical translation that is unimportant for
parameter estimation, the modified log--likelihoods (here with $NE=0.7$) tend to
have a larger maximum close to the supervised estimate (black `x') and, hence,
also to the true parameter value, which will thus tend to also be the global
maximum, while the other local maxima are suppressed. The magnitude of these
effects increase with increasing contextual negentropy, as shown in Figure
\ref{fig:liks}b, where with contextual negentropy approaching 1 (dotted lines)
the problem reduces to supervised learning. In our example, this suppression
allows all context--aware methods to ``escape", in contrast to the \emph{US}
method, the local maximum of \emph{US} on the right side of the initial value
and converge to the first local maximum on the left side of the initial value
(signified with `x' of the respective color). The latter is much closer to the
true parameter value thus, yielding lower estimation bias and less sensitivity
to the initial parameterization, two points where the conventional \emph{US}
training is known to perform poorly.

It is easy to see that the boosting of a contextually enhanced $logL$
(comparative to the equivalent for \emph{US}) close to the supervised local
maximum and the suppression of $logL$ for regions of the parameter space further
away, follows directly from the redistribution of the soft mixture assignments
for each sample achieved in favour of the ``correct" mixture thanks to the
probabilistic labels (as long as the latter indeed points to the correct mixture
for each sample). This refined distribution of confidence in the definitions of
both $logL$ and the E--step is thus the basic operational principle of
context--aware learning methods and the observed effects should generalize for
any type of FMM. Note that for ``correct" context and $NE>0$, method \emph{WCA}
will always yield a more favourable redistribution, while for method \emph{CA}
this will be only true when $p_{ij}>\pi_j$ for some sample $\bs{x_i}$ with
$y_i=j$. However, for most estimation problems where the expectations
$\mathbb{E}_{\bs{\hat{\theta}}}\{z_{ij}\}$ will tend to be close to uniform,
improvement should be expected also for most samples with the \emph{CA} case,
especially as $NE$ is increased.

The improvement of convergence rate and its dependency on contextual negentropy
are also evident in the example, since the estimates $\hat{\mu_1}^1$ for
\emph{CA} (blue `o') and \emph{WCA} (green `o') are much closer to their final
MLE than for \emph{US} (red) or \emph{CAE} (\emph{CA} with ignorant context,
magenta) already after the first iteration. This fact is further substantiated
in the next section. It is also interesting to note that method \emph{DCA},
though it still yields a better estimate than \emph{US} started from this
initial point, results in a larger bias than the other context--aware methods,
suggesting that discarding BU information is suboptimal. In fact, one can easily
see that \emph{US} started from an initial point closer to 1 would yield a
better MLE than \emph{DCA} (which is independent of initial estimates as it does
not belong to the EM framework). Finally, in the case of ignorant context
($NE=0$) method \emph{WCA} (solid green line, Figure~\ref{fig:liks}b) reduces to
a translated version of \emph{US} (red), while \emph{CA} (blue) already
``boosts" the favourable maximum, suggesting that \emph{CA} is to be preferred
for context with low $NE$, at least in the case that mixing proportions $\pi_j$
are known.

\subsection{Missing information principle, standard errors and convergence
rate}
\label{subsec:frac}
The application of the \emph{missing information principle} (MIP) on methods
\emph{CA, WCA, US} is demonstrated in a two-mixture of univariate Gaussians
problem with $\pi_1=0.6,\mu_1=0,\mu_2=1,s_1=1,s_2=2$, where standard deviations
are fixed and $\pi_1,\mu_1,\mu_2$ are estimated from initial guesses
$\hat{\pi_1}^0=0.5,\hat{\mu_1}^0=0.49,\hat{\mu_2}^0=0.51$. For increasing values
of contextual negentropy $NE$, we perform 100 repetitions randomly generating
$N=10^4$ samples from the above distribution and estimate the standard errors of
parameters $\pi_1,\mu_1,\mu_2$ and the algorithm's convergence rate as
theoretically predicted by means of estimating the corresponding observed
information matrix for each method (see Section \ref{subsec:mip}). For a certain
contextual negentropy value, a final standard error for each parameter and a
convergence rate value is derived by averaging across the 100 repetitions.

\begin{figure}[h!]
  \centering
  \includegraphics[width=\textwidth]{img/Figure2.pdf}
  \caption{(a) Average predicted standard errors of $\hat{\pi_1}$ ($\Diamond$),
    $\hat{\mu_1}$ ($\triangledown$) and $\hat{\mu_2}$ ($\square$) and their sum
    ($\circ$) with increasing contextual negentropy $NE$ in 100 repetitions of a
    two--mixture of Gaussians estimation problem (see text). Different methods
  color--coded in the legend. (b) Average predicted convergence rates and their
standard deviations for the three methods (color--coded in the legend) in the
same estimation problem.}
  \label{fig:se_conv}
\end{figure}

Figure~\ref{fig:se_conv}a illustrates the average predicted standard errors of
estimates $\hat{\pi_1}$ ($\Diamond$), $\hat{\mu_1}$ ($\triangledown$) and
$\hat{\mu_2}$ ($\square$) as well as their sum ($\circ$) with increasing
contextual negentropy $NE$ for \emph{US} (red), \emph{CA} (blue) and \emph{WCA}
(green). A first important result is that standard errors of all parameters, as
well as their sum, decrease with increasing negentropy for both methods that
employ contextual assistance towards a parameter--specific limit, while they
remain stable for regular unsupervised estimation, thus showcasing a significant
benefit of employing context for parameter estimation. Furthermore,
Figure~\ref{fig:se_conv}b shows that in the same problem, the convergence rate
$r^{\prime}$ of \emph{CA} (blue) and \emph{WCA} (green) is improved with
increasing contextual negentropy to reach immediate convergence ($r^{\prime}=1$,
single iteration) in the case of context fully revealing the missing labels
($NE=1$).

Figure~\ref{fig:mip} reveals the mechanism through which contextual assistance
achieves the aforementioned improvements as a result of the MIP. Recall that, as
discussed in Section~\ref{subsec:mip}, standard errors are the square roots of
the diagonal elements of the MLE variance-covariance matrix $C=I^{-1}$, where
$I=I_c-I_m$ the observed information matrix, $I_c$ the observed complete--data
information matrix and $I_m$ the observed missing information matrix, while the
convergence rate is the spectral radius of the rate matrix $J=I_c^{-1}I_m$,
expressing the fractions of missing information across all estimated parameters.
All the above matrices are evaluated at the MLE after the algorithm has
converged.

\begin{figure}[h!]
  \centering
  \includegraphics[width=\textwidth]{img/Figure3.pdf}
  \caption{Information matrices $I_c$, $I_m$ and rate matrix $J=I_c^{-1}*I_m$
    with increasing contextual negentropy $NE$ in a two--mixture of Gaussians
    estimation problem (see text), for \emph{WCA} (a) and \emph{CA} (b). All
    matrix values normalized to $[-1,1]$ by dividing with the respective
    absolute value of the \emph{US} method.}
  \label{fig:mip}
\end{figure}

For one repetition of the same problem, Figures~\ref{fig:mip}a (for \emph{WCA})
and \ref{fig:mip}b (for \emph{CA}) show that matrix $I_c$ remains unaffected by
increasing context, which is reasonable since the complete--data information
estimates assume data labels known, while the magnitudes of the missing
information matrix elements are reduced with increasing contextual negentropy to
eventually vanish into the 0 matrix as $NE\rightarrow1$. Consequently, the
fractions of missing information (rate matrix) also vanish, leading the largest
eigenvalue of $J$ to gradually approach 0 and hence the global rate of
convergence to 1. In other words, this analysis theoretically establishes what
is intuitively expected: context--aware EM methods improve FMM parameter
estimation by eliminating the missing label information to a certain degree
depending on the contextual negentropy. 

Additionally, the application of the MIP proves that context--aware methods will
operate somewhere in the middle of the unsupervised and supervised extremities:
employing ignorant labels ($NE=0$), yields $I_m^{WCA}=I_m^{US}\Rightarrow
I^{WCA}=I^{US}$ (see below for \emph{CA}) and $I_m^{WCA,CA}=0$ for $NE=1$, thus
the information matrix $I^{WCA}$ coincides with that of \emph{US} for ignorant
context. Conversely, $I^{WCA}=I^{CA}=I_c$ holds for ``perfect context", yielding
in this case the same standard errors (the limits towards both \emph{CA} and
\emph{WCA} methods converge to in our example, Figure~\ref{fig:se_conv}) and
convergence rates of supervised learning.  In Appendix~\ref{app:infomat} we
formally prove that this result generalizes for any FMM parameter estimation
problem.

A second important result regards a notable difference between \emph{CA} and
\emph{WCA}. As shown in Figure~\ref{fig:se_conv}, standard errors and
convergence rates of \emph{CA} demonstrate a superiority over \emph{WCA},
starting from a better point at $NE=0$ and remaining better than the \emph{WCA}
equivalents for the largest part of $NE$ spectrum, until, as discussed, both
methods converge to the supervised estimates at $NE\rightarrow1$. While standard
error of $\mu_1$ is an exception in our particular example, this rule always
holds for the sum of standard errors of all parameters in an FMM estimation
problem. 

The explanation of this effect can be found in the form of the complete--data
log--likelihoods and the E--step formulations of Table~\ref{tab:methods}; while
the structure of the observed information matrices is identical for \emph{WCA}
and \emph{US} for the same parameter estimation problem (the numerical
differences are not associated to the matrix structures, but to their evaluation
at a different MLE with different expectations
$\mathbb{E}_{\bs{\hat{\theta}}}\{z_{ij}\}$ as denoted by the differences in the
formulations of the E--step for the two methods), the structure of the matrices
for \emph{CA} are \emph{reduced} by removing the rows and columns corresponding
to the mixing coefficients $\pi_j,\forall j$ (Figure~\ref{fig:mip}b, row and
column for $\pi_1$ are deleted). This comes from the definitions of $I_c, I_m$
on the respective complete--data log--likelihoods, since mixing coefficients are
missing from the relevant expressions of \emph{CA}. 

The improvements in terms of standard errors and convergence rates hence come as
a result of removing in the \emph{CA} case the missing information associated
with mixing coefficients $\pi_j$, thus leading to a lower total fraction of
missing information for the internal parameters of the mixtures in the \emph{CA}
case than that of \emph{WCA} even for the same level of contextual assistance
$NE$\footnote{In repeated simulations with different mixture types and estimated
  parameters, we find that eigenvalues $\lambda_i,i=1,\dots,N$ of a rate matrix
  $J$ in a problem of $N$ estimated parameters and the eigenvalues
  $\rho_i,i=1,\dots,N-1$ of the reduced matrix $J^{\prime}$ resulting from $J$
  by deleting any $j^{th}$ row and column associated with parameter $\theta_j$
  being fixed to a known value, respect an eigenvalue interlacing property
  $\lambda_k\geq \rho_k \geq \lambda_{k+1}$. Regarding the largest eigenvalues
  of the two rate matrices, this means that fixing a parameter for a given EM
  FMM estimation problem can only improve the global rate of convergence.
  However, a formal proof cannot be easily established for rate matrices since
  in general they do not respect any particular form where this property is
known to hold.}. An exception occurs in problems where mixing coefficients are
known, sine in that case both methods yield the same reduced structure of
information matrices. It should be mentioned that parameters $\pi_j$ can still
be computed in the \emph{CA} case independently as
$\pi_j=\sum_{i=1}^{N}\mathbb{E}_{\bs{\hat{\theta}}}\{z_{ij}\}/N$ after the rest
of the parameters $\bs{\theta}$ have been estimated through EM, and the
associated observed information matrix $I^{\pi}=I^{\pi}_c$ pertaining to the
mixing coefficients can be established through the definition of the
complete--data log--likelihood of $\pi_j$s as
$logL_c^{\pi}=\sum_{i=1}^{N}\sum_{j=1}^{M}\mathbb{E}_{\bs{\hat{\theta}}}\{z_{ij}\}\log{\pi_j}$.
The same holds for method \emph{DCA} (not shown here) operating outside the EM
framework, by applying the definition of $I_c$ on the respective complete--data
log--likelihood in Table~\ref{tab:methods}. The latter method generally yields
better standard error estimates than all other methods and converges in a single
iteration, but as already implied in the previous section and further justified
later on, suffers large estimation imprecision.

The distribution of the remaining amount of missing information across the
internal mixture parameters can vary for methods \emph{CA} and \emph{WCA},
therefore it is not guaranteed that all parameters will yield lower standard
errors in the \emph{CA} case (e.g. $\mu_1$ in our example). However, it is
guaranteed that since the total fraction of missing information is reduced, the
sum of standard errors of all estimated parameters will be lower in \emph{CA}.
Similarly, since the global (for all parameters) and componentwise rates of
convergence only depend on the total fraction of missing information (except
cases rarely occurring in practice, where different components can converge at
different rates, see \citep{Meng94}), the rate of convergence of \emph{CA} is
guaranteed to be higher than that of \emph{US} and \emph{WCA} for a given $NE$.
The latter is also experimentally verified, since the measured global and
componentwise convergence rates coincide with one another and with the
theoretical predictions in all our simulations.

\subsection{Extension to arbitrary cases}
\label{subsec:res_gen}

In Appendix~\ref{app:infomat}, it is shown that the conclusions of the previous
section should generalize to arbitrary FMM cases. We experimentally verify the
applicability of the MIP in four different scenarios: a two--mixture of
Maxwell--Boltzmann distributions (to show the applicability of MIP in a mixture
type different than the common normal distribution, which, additionally, does
not belong to the regular exponential family), a two--mixture of univariate
Gaussians estimating all existing parameters (extension to arbitrary number of
parameters), a three--mixture of univariate Gaussians (extension to arbitrary
number of mixtures) and a two--mixture of multivariate (2D) Gaussians (extension
to the multivariate case). In all the above scenarios, all existing parameters
for each problem are estimated, in 100 repetitions of $N=3\times10^4$ samples.
High separability and initial estimates close to the true values have been
selected to ensure that all methods, including \emph{US}, converge to a local
maximum and the evaluation of information matrices (and hence convergence rates
and standard errors) is sound for all the examined problems\footnote{Exceptions
  to the convergence of an EM algorithm to a local maximum occur when the
  spectral radius of $J$ exceeds unity, implying the existence of a ridge in the
  incomplete--data log--likelihood. In this case, standard error estimates and
  convergence rates predicted through the evaluation of information matrices
  will not coincide with the measured values.  In a problem converging to a
  local maximum, all eigenvalues of $J$ lie in $[0,1]$ if $I_c$ is positive
  semi--definite or $[0,1)$ if $I_c$ is positive definite, see
  \citep{McLachlan08}}.

\begin{figure}[h!]
  \centering
  \includegraphics[width=\textwidth]{img/Figure4.pdf}
  \caption{(a) Average (across repetitions) of standard error sums (across all
    parameters) in a two--mixture of Maxwell-Boltzmann distributions ($\circ$),
    a two--mixture of univariate Gaussians ($\square$), a three--mixture of
    univariate Gaussians ($\triangledown$) and a two--mixture of 2D multivariate
    Gaussians($\Diamond$) with increasing contextual negentropy $NE$ in 100
    repetitions for each $NE$ level (see Section~\ref{subsec:res_gen}).
    Different estimation methods color--coded in the legend. (b) Average
  predicted convergence rates for the three methods (color--coded in the legend)
in the same estimation problems.}
  \label{fig:se_conv_gen}
\end{figure}

Figure~\ref{fig:se_conv_gen} confirms that the conclusions of the previous
section apply in all the examined case studies. One might also note that
important improvements of standard errors and convergence rates are obtained
even for low $NE$. This implies that it is worth to employ context--aware
methods even in case the confidence of probabilistic labels that can be
retrieved in a particular application is not very high. Additionally, it should
be noted that, especially for the case of three Gaussian mixtures, a very
``easy" problem had to be selected to ensure convergence of \emph{US} and even
\emph{WCA} for all repetitions. This implies that beyond the advantages of
\emph{CA} in regular problems, it is even more important that \emph{CA} is able
to turn irregular problems (where the other methods fail to converge to a local
maximum) into regular ones.

\subsection{Estimation fitness}
\label{subsec:kl}

Having established the benefits brought forward by context--aware methods
regarding convergence rates and standard errors, we move to examine any
estimation fitness improvements achieved by these methods. Towards this goal,
the KLDS fitness criterion introduced in Section~\ref{subsec:metrics} is used in
different estimation scenarios.

\begin{figure}[h!]
  \centering
  \includegraphics[width=\textwidth]{img/Figure5.pdf}
  \caption{Parameter estimation fitness as KLDS in (a) a two--mixture of
    Maxwell-Boltzmann distributions, (b) a two--mixture of univariate Gaussians,
    (c) a three--mixture of univariate Gaussians and (d) a two--mixture of 2D
    multivariate Gaussians with increasing contextual negentropy $NE$ in 100
  repetitions for each $NE$ level (see Section~\ref{subsec:kl}). Different
estimation methods color--coded in the legend.}
  \label{fig:kl_easy}
\end{figure}

Figure~\ref{fig:kl_easy} illustrates the overall estimation fitness as KLDS for
the same ``easy" estimation problems (with the same settings) of the previous
section. All methods are shown to provide close to perfect estimation (true
parameter values recovered and $KLDS\approx0$), with the exception of
\emph{DCA}, which only performs well with strong contextual assistance
($NE\rightarrow 1$) as a result of discarding BU information. Consequently, this
method should be only employed when fast computation is required and
high-confidence probabilistic labels can be retrieved and is excluded hereby
from any further analysis. All context--aware methods converge to the supervised
learning parameter values (which are very close to the true parameter values as
high $N$ has been used) for $NE=1$, as expected.

It is also apparent that in such ``easy" problems, where a local maximum exists
close to the true parameter values for all methods and the initial conditions
are close enough to this maximum, one has nothing to gain concerning estimation
precision by employing context--aware methods. In fact, as also happens in the
simple example of Figure~\ref{fig:liks}, this favourable  local maximum for
\emph{US} is closer to the true parameter values than for the other methods,
yielding better KLSD for method \emph{US} (especially when \emph{CA, WCA}
operate at low $NE$). In conclusion, the benefits of context--awareness in terms
of estimation fitness are only obvious for ``harder" problems, where multiple
local maxima exist and sensitivity to initialization can have a large effect on
estimation precision. 

Note, however, that even in this case, since estimation fitness of \emph{CA} and
\emph{WCA} is still close to optimal, the superiority of these methods in terms
of convergence rate and standard errors could still be strong motivations to
justify their employment instead of \emph{US}. Furthermore, it is only in rare
situations that one has beforehand good knowledge of whether a certain
initialization is a good choice, a problem usually treated with tedious repeated
estimation with different random initializations.

Another interesting observation regards the slightly compromised KLDS of
context--aware methods (in comparison to \emph{US}) for all problems at low $NE$
levels. Inspection of the different terms of the KLDS criterion reveals that in
all cases this effect is due to imprecision in the estimation of the mixing
coefficient distribution $\bs{\pi}$, while the internal mixture parameters
converge very close to their true values, in what appears to be a trade--off on
estimation fitness across these two types of parameters for context--aware
methods. This issue is investigated in Appendix~\ref{app:mixcoef}.
\begin{figure}[h!]
  \centering
  \includegraphics[width=\textwidth]{img/Figure6.pdf}
  \caption{Parameter estimation fitness as KLDS in two--mixture of univariate
    Gaussian problems, where the euclidean distance of the true mixture means
    $D=|\mu_1-\mu_2|$ is increased from $0.01$ to $0.5$ centered at $0.5$, and
    the initialization of means is kept stable to $\mu_1^0=\mu_2^0=0.5$ (see
  Section~\ref{subsec:kl}). \emph{US} method and negentropy levels $NE=0, 0.1,
1$ shown for (a) \emph{CA} and (b) \emph{WCA} as color--coded in the legends.
(c) Average KLDS and standard deviations in 100 repetitions with random
initialization for problem with $D=0.5$.}
  \label{fig:kl_hard}
\end{figure}

Figure~\ref{fig:kl_hard} confirms that improvements in estimation fitness should
be in general expected for common, ``harder" problems with multiple local
maxima; six different two--mixture of univariate Gaussian problems are generated
with $\pi_1=0.5,s_1=0.8,s_2=1.2$, where the distance between the true mixture
means is varied as $D=|\mu_1-\mu_2| \in \{0.01,0.1,0.2,0.3,0.4,0.5\}$ centered
at $0.5$ and the initialization is kept constant as
$\pi_1^0=0.4,s_1^0=s_2^0=1,\mu_1^0=\mu_2^0=0.5$. 100 repetitions for each of the
6 problems are executed with $N=10^4$ and all contextual negentropy levels are
tested for each repetition. The average KLDS values for \emph{US} and
$NE=0,0.1,1$ for methods \emph{CA} and \emph{WCA} after convergence for each
repetition are reported in Figure~\ref{fig:kl_hard}a--b (standard deviations
across repetitions were found to be negligible and are omitted for clarity of
presentation).

In these cases it can be seen that with the exception of \emph{WCA} with $NE=0$
which has been theoretically shown above to be identical to \emph{US}, important
improvements in estimation precision are achieved by context--aware methods even
for low $NE$. This comes as a result of \emph{US} getting ``stack" for the
different problems to some local maximum close to the constant initialization
point, while context--aware methods (for \emph{CA}, even with ignorant context
$NE=0$) are able to adequately suppress those unfavourable maxima and converge
to one closer to the true parameter values, much like it is shown in the simpler
example of Figure~\ref{fig:liks}. For $NE=1$ both context--aware methods
converge to the supervised estimate which is naturally very close to the true
parameter values yielding an almost 0 KLDS. It is also interesting to note that
in this case the gains in terms of estimation precision tend to be greater as
the problem becomes ``easier" (means are dragged farther apart); this effect
however is specific to the particular example and should not generalize, since
it is attributed to the fact that the local maximum towards which \emph{US} gets
stack is always close to the initial values and thus farther away from the true
parameters $\mu_1,\mu_2$ as the latter are dragged more and more apart. In any
case, the ``separability" of the mixtures does not seem to play an important
role on the expected improvements from context--aware methods.

In order to verify the latter conclusions and investigate the comparative
sensitivity of context--aware methods to initialization, we generate 100
repetitions of the problem with $D=0.5$, where the initial parameter guesses are
randomly selected from uniform distributions $\pi_1^0 \in [0.1,0.9]$,
$\mu_1^0,\mu_2^0 \in [-2,2]$ and $s_1^0,s_2^0 \in [0.5,2]$.
Figure~\ref{fig:kl_hard}c shows that estimation precision of \emph{US} with
random initialization for problem with $D=0.5$ is on average lower than that
achieved with the constant initialization used for
Figures~\ref{fig:kl_hard}a--b, thus implicitly confirming that increasing KLDS
for \emph{US} with larger $D$ is simply the effect of the constant 
initialization imposed in the previous simulation.   

Most importantly, methods \emph{CA} and \emph{WCA} (for $NE>0$) are shown to
yield lower KLDS average and standard deviation, proportionally to $NE$ (for
$CA$ even with ignorant context $NE=0$), proving that context--aware methods
will be less sensitive to initialization thanks to suppression of unfavourable
local maxima and the ``boosting" of the local maximum closer to the supervised
estimate, as shown in the Figure~\ref{fig:liks}b. An important disadvantage of
regular unsupervised learning can be thus attenuated or even completely
alleviated through context. Furthermore, it is shown that the demonstrated
superiority of method \emph{CA} over \emph{WCA} in terms of convergence rate and
standard errors extends to estimation precision. Another important result is
that, since \emph{CA} with ignorant context has been shown to yield lower
standard errors, larger convergence rate and better estimation precision, it is
worth to avoid estimating the mixing coefficients altogether, even in the
regular unsupervised case (unavailable context).

\begin{figure}[h!]
  \centering
  \includegraphics[width=\textwidth]{img/Figure7.pdf}
  \caption{(a) Class--bias as $D_{KL}(f_1^A||f_1^E)-D_{KL}(f_2^A||f_2^E)$ in
    estimation problems with unbalanced number of samples. (b)
    $KLDS_{CA,WCA}-KLDS_{US}$ against contextual negentropy $NE$ and percentage
    of erroneous context $\alpha$. (c) KLDS in a ``mixed"-- and low--context
  simulation. See text for details.}
  \label{fig:kl_bwm}
\end{figure}

It can be reasonably suspected that the provision of assistance in the form of
probabilistic labels might also help to cope with situations where the training
datasets are classwise unbalanced and the estimation problem is inherently
``biased" towards the dominant class. To investigate the effects of methods
\emph{CA, WCA} in this aspect, the actual underlying parameter $\pi_1$ in the
same two--mixture of Gaussians problem (with $\mu_1=0, \mu_2=1$) is modified
taking values in $[0.2,0.8]$ (consequently, also the proportion of generated
samples belonging to the first mixture is altered accordingly) and 100
repetitions with $N=10^4$ and random initialization (in the same fashion as for
the previous simulation) are executed for each $\pi_1$ value tested.
Figure~\ref{fig:kl_bwm}a shows the average difference $D_{12} =
D_{KL}(f_1^A||f_1^E)-D_{KL}(f_2^A||f_2^E)$ color--coded as shown in the
colorbar. The fading blue color of method \emph{US} (first row) illustrates that
this particular problem is inherently biased in favour of the first mixture,
which is not surprising since $s_1<s_2$. However, as expected, this bias
diminishes as more samples of the second mixture are generated at the expense of
the first mixture ($\pi_1 \in [0.2, 0.4]$). Furthermore, as also shown above,
both context--aware methods are able to completely eliminate bias as a result of
generally reducing the overall KLDS for context with high negentropy $NE \in
[0.5,0.99]$. It is more interesting to observe the effect of context--awareness
for low negentropy context; \emph{CA} is shown to regulate class--bias
proportionally to $\pi_1$ with ignorant context $NE=0$ (thus redistributing the
imprecision of estimation evenly across mixtures), while it largely eliminates
estimation bias already at $NE=0.1$ and thereafter.  Conversely, \emph{WCA}
performs identically to \emph{US} for $NE=0$ (a result already established
above), and redistributes the bias proportionally to $\pi_1$ for low $NE$,
instead of eliminating it. Hence, method \emph{CA} seems to be also dominant
concerning bias elimination in unbalanced problems.

Using the same estimation problem as testbed, the effect of erroneous context is
evaluated by imposing a percentage $\alpha \in [10, 90]\%$ of ``wrong"
probabilistic labels assigned randomly to the $N=10^4$ generated samples. 100
repetitions are executed for each tested $\alpha$ value with random
initialization. Figure~\ref{fig:kl_bwm}b illustrates the average difference
$KLDS_{CA,WCA}-KLDS_{US}$ for different $\alpha$ and $NE$ color--coded as shown
in the respective colorbar. As expected, for ignorant context $NE=0$, \emph{WCA}
yields identical estimation precision to \emph{US}, while \emph{CA} yields
slight improvements when $\alpha \approx 50\%$. For low $NE \in [0, 0.3]$ and a
majority of wrong probabilistic labels, $\alpha \in [60, 90]$, context is shown
to be particularly detrimental since it will tend towards the ``reverse" of the
actual mixture parameter values, showing that these methods should not be
employed in case the derived contextual assistance has a probability of being
wrong which is larger than 0.5. It is surprising that even for $\alpha > 50 \%$,
increasing contextual negentropy seems to attenuate the negative effects of
prevailing erroneous context, for both methods. Finally, it is shown that
starting with $\alpha = 50\%$ and especially as $\alpha \rightarrow 0$ and $NE
\rightarrow 1$ the estimation fitness becomes significantly better than
\emph{US}. Overall, it seems that ``wrong" context is not essentially
detrimental as long as correct probabilistic labels are prevailing, thus the
proposed context--aware methods can be employed even when one cannot assure
absolutely accurate context.  Moreover, the benefits in terms of convergence
rates and standard errors (not shown here) remain unaffected by the existence of
wrong context. The comparative evaluation attempted here depends on the average
KLDS achieved by \emph{US} in this particular problem, thus the percentage of
wrong labels $\alpha$ below which context--aware methods achieve improved
estimation precision is also problem--dependent. Yet, in additional simulations
executed in different scenarios the overall picture suggests that non-prevailing
erroneous context does not counteract the methods' benefits.

In the so far demonstrated simulation experiments, a certain contextual
negentropy value $NE$ is applied to all the probabilistic labels. However, in
real applications it is more likely that one has to cope with retrieved context
of fluctuating (across the acquired data samples) and probably low $NE$. We
investigate the influence of ``mixed"--, wrong-- and low--negentropy
probabilistic labels in the same estimation problem as above, with random
initialization in 100 repetitions where the $\alpha$ \% of the probabilistic
labels are erroneous and the negentropy $NE$ of each label is randomly retrieved
from the uniform distribution $NE \in [0, 0.2]$.  Figure~\ref{fig:kl_bwm}c
verifies that both context--aware methods yield better KLDS than \emph{US} for
$\alpha <= 0.5$, and that this improvement can be achieved despite the ``mixed"
and low negentropy of the provided probabilistic labels. Furthermore, the
convergence rates and standard errors of this simulation were found to be
approximately equal to the equivalent uniform negentropy experiment with $NE =
0.1$. Hence, in ``mixed"--context situations, one can still predict the
performance of context--aware methods using the average $NE$ of the retrieved
contextual probabilistic labels.

\subsection{Online context--aware learning in brain--computer interface}
\label{subsec:bci}

The applicability, efficiency and effectiveness of context--aware learning are
demonstrated in an online--learning problem from the field of brain--computer
interaction (BCI). More specifically, we employ a binary speller which allows a
user to type messages by means of two control commands. The latter are
implemented as a 2-class, motor imagery (MI) BCI, where the BCI translates
processed brain activity patterns as recorded online through
electroencephalographic (EEG) signal into one of the two required application
control commands, as in \citep{Millan08}. The user attempts to spontaneously
generate one of the two desired brain patterns by imagining a corresponding limb
movement (e.g.  right/left hand or feet movement). The motor imagery spelling
paradigm can thus provide computer accessibility to individuals with lost motor
function.

Besides presenting a tough classification problem due to low signal--to--noise
ratio (SNR) of EEG signal, MI BCI is also known to suffer from non-stationarity
of the extracted brain patterns, which renders a previously trained classifier
ineffective (primarily) in--between, or even, during spelling sessions, a
situation so far coped with frequent supervised classifier retraining. This
traditional solution, however, is particularly cumbersome, as it requires
frequent interruptions of spelling efforts where the subject engages into
lengthy and de--motivating supervised training protocols. The same holds for the
subject's initial BCI training phase. Online--learning is a natural solution to
the above problems, yet, it generally has to be carried out in an unsupervised
manner, since in the vast majority of real BCI applications including spelling,
data labels cannot be retrieved during online BCI operation. Consequently,
adaptive, online classifier training in BCI is bound to suffer the known
shortcomings of unsupervised learning, yielding generally inferior estimation
quality compared to supervised retraining protocols. It is thus straightforward
that context--aware learning proposed in this work could allow uninterrupted BCI
spelling largely avoiding the deficiencies of unsupervised learning.

We hereby devise a buffer approach for continuous, context--aware
online--learning of an LDA BCI classifier (estimation of class--dependent mean
vectors and common covariance matrix) as: 

\begin{equation}
  \bs{\mu_j^t}=\frac{N-b_j^t}{N}\bs{\mu_j^{t-1}}+\frac{b_j^t}{N}\bs{\mu_j^{EM}}
\label{eq:on_m}
\end{equation}
\begin{equation}
  \Sigma^t=\frac{N-b^t}{N}\Sigma^{t-1}+\frac{b^t}{N}\Sigma^{EM}
  \label{eq:on_cov}
\end{equation}
\begin{equation}
  \bs{\mu_j^{EM}}=\frac{1}{b_j^t}\sum_{k=t-N+1}^{t}\alpha_k^j\bs{x_k}
\label{eq:mem}
\end{equation}
\begin{equation}
  \Sigma^{EM}=\frac{1}{b^t}\sum_{k=t-N+1}^t\sum_{j=1}^2
  \alpha_k^j(\bs{x_k}-\bs{\mu^t_j})^T(\bs{x_k}-\bs{\mu^t_j})
\label{eq:covem}
\end{equation}
where, $\alpha_k^j=\mathbb{E}_{\bs{\hat{\theta}}}\{z_{kj}\}$,
$b_j^t=\msum{k=t-N+1}{t}\alpha_k^j$ and $b^t=b_1^t+b_2^t$. This type of online
ML learning solves the regular EM FMM iterative learning for a buffer of the
latest $K$ ($K\leq N$) samples $\bs{x_k}$ (M--step in Equations~\ref{eq:mem} and
\ref{eq:covem}), repeating the estimation at each time $t$ when a new sample has
been received from the BCI. The latest sample is added on top of the buffer
stack and, in case the stack is full ($K=N$), the oldest sample at the stack's
bottom is discarded. The final estimates at time $t$ are derived as a weighted
average of the buffer--based EM ML estimates and the previous estimates at $t-1$
(Equations~\ref{eq:on_m} and \ref{eq:on_cov}), adding parsimony to the model.
The entities $b_j^t$ and $\alpha_k^j$ are derived from the last EM iteration on
the buffered samples and the initial estimates used at the first iteration are
$\mu_j^{t-1}$ and $\Sigma^{t-1}$. The overall intensity of adaptation is thus
only controlled by the buffer size $N$ even when only $K < N$ samples have been
collected in the beginning of the experiment. The change in the mean vector
$\bs{\mu_j^t}$ further depends on the estimated number of samples in the buffer
belonging to class $j$, $b_j^t$, thus unbalanced buffers are automatically
handled and the expectations $\alpha_k^j$ (which are the only variables
depending on contextual assistance) influences the adaptation intensity in
addition to precision. 

\begin{figure}[h!]
  \centering
  \includegraphics[width=\textwidth]{img/Figure8.pdf}
  \caption{(a) Speller GUI and (b) underlying binary tree structure in a reduced
  dictionary.}
  \label{fig:bt}
\end{figure}

The employed speller is shown in Figure~\ref{fig:bt}, where an underlying binary
tree structure (Figure~\ref{fig:bt}b) is hidden behind a simple graphical user
interface (GUI, Figure~\ref{fig:bt}a). The available characters are leaf nodes
of the tree, thereby each character is assigned a binary 0/1 (left/right)
codeword, depending on the left/right commands required to reach it from the
tree's root. The current node in the tree is visualized by the red cursor
(caret) and the available characters are surrounded by the orange “bubble”. The
user has to identify the position of the desired character relatively to the
caret, simplified by imposed alphabetic ordering, and forward the appropriate
BCI command (by employing the respective MI task) to move the caret towards it.
A conventional MI feedback bar is embedded into the speller GUI (Figure 1a) to
continuously visualize the user’s intent. A newly acquired EEG sample $\bs{x_t}$
is classified with the LDA classifier estimated at time $t-1$ as belonging to
the left/right class, moving the feedback bar a step towards the respective
direction. A left/right tree descending command is forwarded when the feedback
bar reaches the left/right threshold, and a character is typed when the
respective leaf node is reached, whereby a new binary tree is generated to allow
typing the next character, placing the caret at the root of the new tree.

The above application and online--learning settings are ideal for demonstrating
the applicability and benefits of context--aware learning. A speller has been
also used to test a context--aware discriminative algorithm in
\citep{Kindermans12a,Kindermans12b}. Concerning applicability, a spelling
application offers a natural interpretation and derivation of contextual random
variables $c_t$, which represent the desired character. A commonly used
prefix--based language model provides the necessary contextual prior information
$p(c_t)$, while, the conditionals $p(z_t|c_t)$ are derived automatically through
the knowledge of the current node position in the binary tree structure of the
speller (in this case, $p(z_t|c_t)$ is either 0 or 1, depending only on the
caret position). \emph{CA}--type of learning should be naturally applied, since
the sample class labels $z_t$ (representing the application command the user is
trying to reach and implicitly the MI task/class currently employed) depend on
the desired character $c_t$, and not vice--versa.  The actual $c_t$ is not
observed (the algorithm ignores which character the user is trying to reach,
which fulfills the requirement of non--explicit supervision) therefore, the
definition of probabilistic labels $p_{tj}=\sum_{l=1}^Lp(c_t=l)p(z_j|c_t=l)$ is
employed (see Appendix \ref{app:proofs}). 

We manipulate the average negentropy $NE$ of the retrieved probabilistic labels
by generating the binary trees of the speller through
suboptimal\footnote{Shannon-Fano coding achieves its minimum average code length
  for a 0.5 probability split, still yielding a slightly inferior coding result
  compared to optimal Huffmann coding. A trade--off between maximizing the
  effects of context--aware learning and maximizing the application's efficiency
  exists in this particular spelling application by choosing a 0.9--split, which
  will naturally increase the number of commands needed to reach the desired
  character. This trade-off, however, needs not be the case for general
  applications. For the particular spelling application in question, a
0.5--split can be generally used, switching to a 0.9--split whenever performance
decrease indicates the need for online--learning.} Shannon-Fano coding based on
the distribution $p(c_t)$ provided by the language model, so that the sub-tree
at each hierarchical level yields a probabilistically ``heavy" side of total
probability as close to 0.9 as possible, and a ``light" one on the other side
(the heavy side is reversed at each level). The negentropy of the acquired
probabilistic thus ranges approximately in 0--0.5, with an average close to 0.3. 

\emph{CA}--type of learning is embedded in the algorithm of
Equations~\ref{eq:on_m}--~\ref{eq:covem} through variables $\alpha_k^j$ (recall
that all context--aware methods proposed in this work only affect the E--step of
EM learning). Beyond the expected parameter estimation improvement due to the
illustrated suppression of local maxima, an additional reason why improved
estimation can be expected concerns the computational constraints of
online--learning: the BCI in question operates at 2 Hz, thus leaving 0.5 seconds
within which all necessary operations (preprocessing, feature extraction,
classification and parameter re-estimation) need to be executed. For this
reason, the EM algorithm on the buffer is only allowed to perform as many
iterations as can be executed within 100 msec. Since context--aware learning of
increasing negentropy has been shown above to yield larger convergence rates, it
can be expected that \emph{CA}--learning will also yield more precise estimates
because it has larger chances of converging to the maximum within the given
time. Consequently, we expect the contextually--enhanced algorithm to be faster
and more accurate in estimating a subject's underlying brain activity patterns
leading to faster and improved restoration of a subject's BCI performance in
case of non-stationarities.

We conduct spelling simulations using EEG MI data of 12 subjects recorded in the
lab. For each subject, a common subject--inspecific classifier (trained on MI
data of several other subjects depending on the pair of MI tasks employed by
each subject) is used as the initial point of adaptation. This setting simulates
the initial subject training phase where we investigate the possibility to allow
a subject to immediately engage with device operation, skipping supervised
training altogether. It also simulates situations where an older
subject-specific classifier does not accurately reflect the subject's generated
signals in the new BCI spelling session, as it is often the case. For each
subject, the same spelling task of typing the words ``nothing" and ``portion" is
repeated for the supervised case (true data labels used), the \emph{CA} case
with variable $NE$ as explained above and the \emph{CA} with ignorant context
(constant $NE=0$). The words have been selected so that in the majority of cases
the probabilistic labels of samples point to the ``correct" data classes. The
overall learning problem tested here is that of ``mixed"--context \emph{CA}
learning with a small percentage of ``wrong" context.

The only free parameter of the online--learning algorithm is the buffer size
$N$, which is set hereby to $N=240$ samples, resulting (due to the feature
extraction rate of 2 Hz) in using the last 2 minutes of a subject's MI to
re--estimate the classifier. This buffer size value provides a good trade--off
between estimation stability and fast convergence to the fluctuating brain
patterns. 6--dimensional feature vectors $\bs{x_t}$ are extracted (after
relevant signal processing and spatial filtering) consisting of the signal's
power spectral density in bands $8-14$ Hz and $18-24$ Hz (known to be relevant)
on three cortical locations (EEG channels). A total of 48 parameters has to be
re--estimated at each time $t$, posing a demanding estimation problem where
method \emph{US} was found to perform poorly.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.8\textwidth]{img/Figure9.pdf}
  \caption{Mean and standard deviation of running classification accuracy
  during the spelling tasks for all subjects with supervised estimation and
methods \emph{CA} and \emph{CA--0}.}
  \label{fig:bci}
\end{figure}

We calculate running classification accuracy in a window of the latest minute
(120 samples) of simulated BCI operation, with a shift of 0.5 second (1 sample).
Figure~\ref{fig:bci} shows the means and standard deviations of running accuracy
after the first minute of online--learning with the speller until the end of the
spelling task, for all subjects and methods. The large standard deviations of
running accuracy even for the case of supervised learning (blue bars) reflect
the fact that brain patterns are intensively non--stationary for all subjects.
Yet, with the exception of subject s5 and s8, \emph{CA} learning (green) is
shown to be able to quickly recover from the naive initial classifier estimate,
yielding similar classification accuracy to the supervised case, which
implicitly defines an upper bound of the estimation fitness and classification
accuracy that can be achieved for this particular problem and each subject
regarding the missing label information. Classification results of \emph{CA} are
significantly better than for the ignorant--context \emph{CA} method (red),
which is close to chance level for most subjects. The latter was found to
demonstrate only marginally better results than the regular \emph{US} method
(not shown), representing the unsupervised extremity. 

The case of subject s5 (the only subject in our study that suffers severe motor
impairments), where all methods perform close to chance level, was found to be
due to intense instabilities of the generated brain patterns. Furthermore,
\emph{CA-0} for subject s3 demonstrates a class--inversion effect, which is
attributed to the fact that although this subject is able to generate
discriminant and fairly stable brain patterns, method \emph{CA-0} cannot escape
the local maximum close to the initialization point throughout the spelling
session. On the contrary, in the cases of subjects s1 and s8, initialization is
coincidentally favourable, thus \emph{CA-0} is only slightly inferior (though
still the difference is statistically significant). Note that, a certain level
of single--sample accuracy in MI BCIs translates to a larger command delivery
accuracy thanks to the evidence accumulation of consecutive classification
decisions that happens on the BCI feedback level. In fact, even 60\%
single--sample accuracy is enough for successful (albeit slow) operation of the
speller.

It should be noted that the relative performance of \emph{CA-0} could be
enhanced by either increasing the buffersize $N$ (in order to increase the ratio
of number of samples over the number of parameters) or imposing constraints
which would lead to less estimated parameters, as in \citep{Vidaurre10}. Both
alternatives, however, suffer certain limitations. In the former case, a larger
estimation buffer would compromise the ability of the algorithm to converge fast
to intensively fluctuating brain patterns. In the latter case, reducing the
number of parameters yields a less powerful classifier for all learning methods.
Context--awareness can achieve classification improvement avoiding such
limitations. 

Overall, the above example showcases the possibility to intuitively apply
context--aware parameter estimation in real--world applications involving tough
classification and, possibly, online--learning problems, where the demonstrated
combined benefits in EM MLE parameter estimation (faster convergence rate,
suppression of unfavourable local maxima, less sensitivity to initialization,
operation close to the supervised case) yield a significantly improved
classification outcome without explicit supervision or otherwise manual labour
to collect data labels. From the practical point--of--view, in the particular
application in question, a BCI--speller user will be able thanks to
context--aware learning to communicate at will avoiding retraining sessions that
render the overall BCI application impractical.

